Exploiting Audio-Visual Features with Pretrained AV-HuBERT for Multi-Modal Dysarthric Speech Reconstruction

Dysarthric speech reconstruction (DSR) aims to transform dysarthric speech into normal speech by improving the intelligibility and naturalness. This is a challenging task especially for patients with severe dysarthria and speaking in complex, noisy acoustic environments. To address these challenges, we propose a novel multi-modal framework to utilize visual information, e.g., lip movements, in DSR as extra clues for reconstructing the highly abnormal pronunciations. The multi-modal framework consists of: (i) a multi-modal encoder to extract robust phoneme embeddings from dysarthric speech with auxiliary visual features; (ii) a variance adaptor to infer the normal phoneme duration and pitch contour from the extracted phoneme embeddings; (iii) a speaker encoder to encode the speaker's voice characteristics; and (iv) a mel-decoder to generate the reconstructed mel-spectrogram based on the extracted phoneme embeddings, prosodic features and speaker embeddings. Both objective and subjective evaluations conducted on the commonly used UASpeech corpus show that our proposed approach can achieve significant improvements over baseline systems in terms of speech intelligibility and naturalness, especially for the speakers with more severe symptoms. Compared with original dysarthric speech, the reconstructed speech achieves 42.1\% absolute word error rate reduction for patients with more severe dysarthria levels.

==> acknowledgement.tex <==
%\section{Acknowledgements}
%\label{sec:acknowledgements}

\textbf{Acknowledgement}: This work is partially supported by 
National Key R\&D Program of China (2020AAA0104500),
National Natural Science Foundation of China (NSFC) (62076144),
%the joint research fund of NSFC-RGC (Research Grant Council of Hong Kong) (61531166002, N$\_$CUHK404$/$15),
and National Social Science Foundation of China (NSSF) (13\&ZD189).



==> related_work.tex <==
\section{Related work}
Our work is related to Context-aware Augmented Deep Embedded Clustering (CADEC) \cite{wu2022self} and Vector Quantized-Variational AutoEncoder (VQ-VAE) \cite{van2017neural}.

\subsection{CADEC}
CADEC is a 
% novel 
two-stage style learning approach from abundant unlabeled plain text in a self-supervised manner.
It leverages an emotion lexicon and uses contrastive learning \cite{chen2020simple} and deep clustering \cite{zhang2021supporting}.
Firstly, it uses contrastive learning to pre-train style embedding to distinguish similar and dissimilar utterances. 
To this end, a similar utterance is created by replacing an emotional word, determined by an emotion lexicon, with a similar one, while the other utterances in the randomly sampled minibatch are treated as dissimilar utterances. 
Then the training samples in style embedding space are clustered by minimizing deep clustering loss, reconstruction loss and contrastive loss together. 
Compared with BERT \cite{kenton2019bert}, CADEC style embedding is more effective in learning styles in addition to content.
We adopt CADEC as our style encoder to predict a more style-related representation from context.

\subsection{VQ-VAE}
VQ-VAE is a powerful representation learning framework that can make effective use of the latent space.
It 
% successfully 
combines the variational autoencoder (VAE) framework with discrete latent representations through a 
% novel 
parameterisation of the posterior distribution of (discrete) latents given an observation.
It can successfully model important features that usually span many dimensions in data space (for example objects span many pixels in images, phonemes in speech, the message in a text fragment, etc.) as opposed to focusing or spending capacity on noise and imperceptible details which are often local.
Many extension models have been proposed, leading to high performance in various tasks \cite{zhao2020improved} \cite{williams2021learning} \cite{wang2019vector}.
% voice conversion, disentangle sub-phone content and global-level speaker characteristics \cite{williams2021learning}
We adopt VQ-VAE as our style extractor to extract the latent style embedding from mel-spectrogram.
